Multi-Agent Chance-Constrained Stochastic Shortest Path with Application to Risk-Aware Intelligent Intersection

In transportation networks, where traffic lights have traditionally been used for vehicle coordination, intersections act as natural bottlenecks. A formidable challenge for existing automated intersections lies in detecting and reasoning about uncertainty from the operating environment and human-driven vehicles. In this paper, we propose a risk-aware intelligent intersection system for autonomous vehicles (AVs) as well as human-driven vehicles (HVs). We cast the problem as a novel class of Multi-agent Chance-Constrained Stochastic Shortest Path (MCC-SSP) problems and devise an exact Integer Linear Programming (ILP) formulation that is scalable in the number of agents' interaction points (e.g., potential collision points at the intersection). In particular, when the number of agents within an interaction point is small, which is often the case in intersections, the ILP has a polynomial number of variables and constraints. To further improve the running time performance, we show that the collision risk computation can be performed offline. Additionally, a trajectory optimization workflow is provided to generate risk-aware trajectories for any given intersection. The proposed framework is implemented in CARLA simulator and evaluated under a fully autonomous intersection with AVs only as well as in a hybrid setup with a signalized intersection for HVs and an intelligent scheme for AVs. As verified via simulations, the featured approach improves intersection's efficiency by up to $200\%$ while also conforming to the specified tunable risk threshold.

==> authors.tex <==
\vspace{-13mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/majid.png}}]%
{Majid Khonji} is an assistant professor in the EECS department at Khalifa University, UAE, and a research Affiliate with MIT Computer Science and Artificial Intelligence Laboratory (CSAIL), USA. He received his MSc degree in Security, Cryptology, and Coding of Information Systems from Ensimag, Grenoble Institute of Technology, France, and PhD in Interdisciplinary Engineering from Masdar Institute, UAE, in collaboration with MIT in 2016. Previously, he was a visiting assistant professor with MIT CSAIL, a senior R\&D technologist in Dubai Electricity and Water Authority (DEWA), and an information security researcher in Emirates Advanced Investment Group (EAIG).
\end{IEEEbiography}

\vspace{-13mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/rashid.jpg}}]%
{Rashid Alyassi} received the B.S. degree in Computer Engineering and the M.S. degree in Computer Science from Khalifa University, UAE, in 2017 and 2020, respectively. Currently, he is a Research Engineer with Khalifa University, UAE. His research interests are centered primarily on Automation, safe planning, and algorithms with applications to Autonomous Vehicles. Also, as part of Khalifa University's AVLab team, he won the Dubai World Challenge for Self-Driving Transport 2021.
\end{IEEEbiography}

\vspace{-13mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/Wolfgang.jpg}}]
{Wolfgang Merkt} received the B.Eng.(Hns) degree in mechanical engineering with management and
the M.Sc.(R) and Ph.D. degrees in robotics and autonomous systems from the University of Edinburgh, Edinburgh, U.K., in 2014, 2015 and 2019, respectively.
He is currently a Senior Researcher at the Oxford Robotics Institute, University of Oxford with I. Havoutis. His research interests include fast learning- and optimization-based methods for planning and control, locomanipulation, and legged robots.
\end{IEEEbiography}


\vspace*{-10mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/areg3.jpg}}]%
	{Areg Karapetyan} received the B.S. degree (with honours) in industrial electronics from National Polytechnic University of Armenia in 2010 and in 2015 the M.S. degree in Computing and Information Science from Masdar Institute, UAE, which was created in collaboration with MIT. He received the Ph.D. degree in Interdisciplinary Engineering from Masdar Institute in 2019. From 2019-2020 he was with the Research Institute for Mathematical Sciences (RIMS), Kyoto, Japan as a post-doctoral researcher. Currently, he is a post-doctoral fellow with Khalifa University, UAE. His research interests are centered primarily on the design and analysis of algorithms, mathematical optimization, computing theory and their practical applications in Autonomous Vehicles and Intelligent Systems.
\end{IEEEbiography}

\vspace{-13mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/Cyrus.jpg}}]
{Xin Huang} received the B.S. degree in Engineering and Computer Science from Harvey Mudd College and the M.S. and Ph.D. degrees in Aeronautics and Astronautics from MIT. During his Ph.D., he worked on trajectory prediction and risk-bounded motion planning, with applications in autonomous driving and aircraft routing. His work on interactive trajectory prediction has been highlighted by MIT News. He has won multiple awards at NeurIPS and CVPR. He is a recipient of the 2021 Qualcomm Innovation Fellowship.
\end{IEEEbiography}


\vspace{-12mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/Sungkweon.jpg}}]
{Sungkweon Hong} received his B.S. and M.S. degrees in air transportation from Korea Aerospace University, South Korea, in 2013 and 2015, respectively. He is currently pursuing the Ph.D. degree with the Department of Aeronautics and Astronautics, MIT. Before joining MIT, he was a Researcher with the Communication, Navigation and Surveillance/Air Traffic Management Team, Satellite Based Augmentation System Research and Development Head Office, Korea Aerospace Research Institute, Daejeon, South Korea. His research interests include risk-bounded conditional planning and its application to risk-sensitive domains such as autonomous driving or aircraft operations.
\end{IEEEbiography}


\vspace{-12mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/jorge.jpg}}]
{Jorge Dias} has a Ph.D. on EE and Coordinates the Artificial Perception Group from the Institute of Systems and Robotics from the University of Coimbra, Portugal. He is Full Professor at Khalifa University, Abu Dhabi, UAE and Deputy Director from the Center of Autonomous Robotic Systems from Khalifa University. His expertise is in the area of Artificial Perception (Computer Vision and Robotic Vision) and has contributions on the field since 1984. He has been principal investigator and consortia coordinator from several research international projects, and coordinates the research group on Computer Vision and Artificial Perception from KUCARS.
Jorge Dias published several articles in the area of Computer Vision and Robotics that include more than 300 publications in international journals and conference proceedings and recently published book on Probabilistic Robot Perception that addresses the use of statistical modeling and Artificial Intelligence for Perception, Planning and Decision in Robots. He was the Project Coordinator of two European Consortium for the Projects "Social Robot" and "GrowMeUP" that were developed to support the inclusivity and wellbeing for of the Elderly generation.
\end{IEEEbiography}


\vspace{-12mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/Brian.jpg}}]
{Brian Williams} received his S.B., S.M, and Ph.D. in Computer Science and Electrical Engineering at MIT, and worked at the Xerox Palo Alto Research Center and NASA Ames Research Center, prior to joining the faculty at MIT. He received a NASA Space Act Award for Remote Agent, the first fully autonomous, self-repairing space explorer, demonstrated onboard the NASA Deep Space One probe in May, 1999. He was a member of the Tom Young Blue Ribbon Team in 2000, assessing future Mars missions in light of the Mars Climate Orbiter and Polar Lander incidents, and is currently a member of the Advisory Council of the NASA Jet Propulsion Laboratory at Caltech. He has won four best paper prizes for his research in diagnosis, qualitative algebras, propositional inference and soft constraints. He is a fellow of AAAI, has served as guest editor of the Artificial Intelligence Journal and has been on the editorial boards of the Journal of Artificial Intelligence Research, and MIT Press.
\end{IEEEbiography}


